New formulas for cup-$i$ products and fast computation of Steenrod squares

Operations on the cohomology of spaces are important tools enhancing the descriptive power of this computable invariant. For cohomology with mod 2 coefficients, Steenrod squares are the most significant of these operations. Their effective computation relies on formulas defining a cup-$i$ construction, a structure on (co)chains which is important in its own right, having connections to lattice field theory, convex geometry and higher category theory among others. In this article we present new formulas defining a cup-$i$ construction, and use them to introduce a fast algorithm for the computation of Steenrod squares on the cohomology of finite simplicial complexes. In forthcoming work we use these formulas to axiomatically characterize the cup-$i$ construction they define, showing additionally that all other formulas in the literature define the same cup-$i$ construction up to isomorphism.

==> sec/legacy.tex <==
%\begin{lemma} \label{l:freeness}
%	Let $\gamma_1 + \dots + \gamma_m$ be the basis representation of a cochain in $C^{-n}(X; \Ftwo)$.
%	Consider $i, j \in \{1, \dots, m\}$ with $i \neq j$ and $x \in X_{n+k}$.
%	Let $\Delta_{n-k}$ be as introduced in \cref{d:cup-i coproducts}.
%	\begin{enumerate}
%		\item If $k \neq 0$ then $(\gamma_i \otimes \gamma_i)\Delta_{n-k}(x) = 0$.
%		\item If $(\gamma_i \otimes \gamma_j)\Delta_{n-k}(x) \neq 0$ then $(\gamma_j \otimes \gamma_i)\Delta_{n-k}(x) = 0$.
%	\end{enumerate}
%\end{lemma}
%
%\begin{proof}
%	Recall that
%	\begin{equation*}
%	\Delta_{n-k}(x) \ = \! \sum_{\substack{U \subseteq \{0, \dots, n+k\} \\ \vert U \vert = 2k}}
%	d_{U^0}(x) \otimes d_{U^1}(x).
%	\end{equation*}
%
%	(1) If $(\gamma_i \otimes \gamma_i)\Delta_{n-k}(x) \neq 0$, then there exists a non-empty $U$ in the sum with $U^0 = U^1$, which is impossible since $U^0 \cap U^1 = \emptyset$.
%
%	(2) If $(\gamma_i \otimes \gamma_j)\Delta_{n-k}(x) \neq 0$ and $(\gamma_j \otimes \gamma_i)\Delta_{n-k}(x) \neq 0$, then there are distinct subsets $V$ and $W$ in the sum such that $V^0 = W^1$ and $W^0 = V^1$.
%	But then $V = V^0 \cup V^1 = W^1 \cup W^0 = W$, which is a contradiction.
%\end{proof}

%Let $X$ be a simplicial complex and $\alpha$ a cochain whose support is the subset $A = \{a_1, \dots, a_m\}$ of $X_n$.
%Denote by $\alpha_i$ the cochain dual of $a_i$ and consider $k \in \{1, \dots, n\}$.



%This condition on the pair $\{a_i, a_j\}$ implies in particular that $a_i \cup a_j = x$ since $d_{U^0}(x) \cup d_{U^1}(x) = x$.

%Let us formalize these observations.
%Let $\widetilde{A}$ be the set of all two-element subsets $\{a_i, a_j\} \subseteq A$ with $a_i \cup a_j \in X_{n+k}$.
%There is a natural map $\pi \colon \widetilde{A} \to X_{n+k}$ sending $\{a_i, a_j\}$ to $a_i \cup a_j$.
%Let $\eval \colon A \to \Ftwo$ be the map sending $\{a_i, a_j\}$ to $1$ if there exist $U \subseteq \{0, \dots, n+k\}$ of cardinality $2k$ such that $\{a_i, a_j\} = \{d_{U^0}(x), d_{U^1}(x)\}$ and let $\eval(\{a_i, a_j\}) = 0$ otherwise.
%Notice that if such $U$ exists then it is unique.
%With this notation we have
%\begin{equation*}
%\beta(x) \ = \! \sum_{\{a_i, a_j\} \in \pi^{-1}(x)} \! \eval(\{a_i, a_j\}).
%\end{equation*}
%We will give a computational characterization of $\eval(\{a_i, a_j\}) = 1$ after introducing some more notation.

%Given a finite totally ordered set $S$, the \textit{position function} $\pos_S \colon S \to \Z$ sends an element $s \in S$ to the cardinality of $\{s^\prime \in S \mid s^\prime \leq s\}$.
%For any $S^\prime \subseteq S$ we write
%\[
%\pos_{S} \big( S^\prime \big) =
%\{\pos_{S} (s^\prime) \mid s^\prime \in S^\prime\}.
%\]
%
%Consider $\{a_i, a_j\} \in \pi^{-1}(x)$, two distinct simplices whose union of simplices $a_{ij} = a_i \cup a_j$ equal to $x$.
%Let $(\ast)$ be the statement that there exist $U \subseteq \{0, \dots, n+k\}$ with $\{a_i, a_j\} = \{d_{U^0}(x),\, d_{U^1}(x)\}$.
%%Notice that is such $U$ exists then it is unique.
%We will now describe a condition equivalent to $(\ast)$ in terms of $\{a_i, a_j\}$ only.
%Denote
%\begin{equation*}
%\overline{a}_{i} = a_i \setminus a_j, \qquad
%\overline{a}_{j} = a_j \setminus a_i, \qquad
%\overline{a}_{ij} = \overline{a}_i \cup \overline{a}_j.
%\end{equation*}
%A necessary condition for $(\ast)$ is that $\pos_{a_{ij}} \colon \overline{a}_{ij} \to \Z$ is an isomorphism onto $U$.
%Slightly abusing notation we define the function $\ind \colon \overline{a}_{ij} \to \Ftwo$ by
%\begin{equation*}
%\ind(v) = \pos_{a_{ij}}(v) + \pos_{\overline{a}_{ij}}(v) \text{ mod }2
%\end{equation*}
%and notice that it fits in the commutative diagram
%\[
%\begin{tikzcd}[column sep=small, row sep=small]
%\overline{a}_{ij} \arrow[rr, "\pos_{a_{ij}}", "\cong"'] \arrow[dr, "\ind"', bend right] & &
%U \arrow[dl, "\ind_U", bend left] \\
%& \Ftwo &
%\end{tikzcd}
%\]
%where $\ind_U$ was introduced in \cref{d:index function}.
%Since for $\varepsilon \in \Ftwo \cong \{0,1\}$ we have $U^\varepsilon = \ind_U^{-1}(\varepsilon)$, condition $(\ast)$ is equivalent to the existence of $U$ with
%\begin{equation} \label{e:pos's equal U's}
%\big\{\pos_{a_{ij}}(\overline{a}_i),\, \pos_{a_{ij}}(\overline{a}_j)\big\} = \{U^0, U^1\}.
%\end{equation}
%Or, equivalently, that the function $\ind \colon \overline{a}_{ij} \to \Ftwo$ is constant on both $\overline{a}_i$ and $\overline{a}_j$ with different values, i.e.,
%\begin{equation*}
%\ind(\overline{a}_i) \xor \ind(\overline{a}_j) = \{0,1\},
%\end{equation*}
%where $\ind(S) = \{\ind(v) \mid v \in S\}$ for any $S \subseteq \overline{a}_{ij}$ and $S \xor S^\prime = S \cup S^\prime \setminus (S \cap S^\prime)$.
%
%\anibal{improve this last paragraph}
%There
%Therefore, for any $x \in X_{n+k}$ we have $\beta(x) = 1$ if and only if the set of pairs $\{a_i, a_j\}$ in $\pi^{-1}(x)$ with $\eval(\{a_i, a_j\}) = 1$ is odd; which is equivalent to the condition $x \in B$.

%Let us formalize these observations.
%Let $\widetilde{A}$ be the set of all two-element subsets $\{a_i, a_j\} \subseteq A$ with $a_i \cup a_j \in X_{n+k}$.
%There is a natural map $\pi \colon \widetilde{A} \to X_{n+k}$ sending $\{a_i, a_j\}$ to $a_i \cup a_j$.
%Let $\eval \colon A \to \Ftwo$ be the map sending $\{a_i, a_j\}$ to $1$ if there exist $U \subseteq \{0, \dots, n+k\}$ of cardinality $2k$ such that $\{a_i, a_j\} = \{d_{U^0}(x), d_{U^1}(x)\}$ and let $\eval(\{a_i, a_j\}) = 0$ otherwise.
%Notice that if such $U$ exists then it is unique.
%With this notation we have
%\begin{equation*}
%\beta(x) \ = \! \sum_{\{a_i, a_j\} \in \pi^{-1}(x)} \! \eval(\{a_i, a_j\}).
%\end{equation*}
%We will give a computational characterization of $\eval(\{a_i, a_j\}) = 1$ after introducing some more notation.
%
%Given a finite totally ordered set $S$, the \textit{position function} $\pos_S \colon S \to \Z$ sends an element $s \in S$ to the cardinality of $\{s^\prime \in S \mid s^\prime \leq s\}$.
%For any $S^\prime \subseteq S$ we write
%\[
%\pos_{S} \big( S^\prime \big) =
%\{\pos_{S} (s^\prime) \mid s^\prime \in S^\prime\}.
%\]
%
%Consider $\{a_i, a_j\} \in \pi^{-1}(x)$, two distinct simplices whose union of simplices $a_{ij} = a_i \cup a_j$ equal to $x$.
%Let $(\ast)$ be the statement that there exist $U \subseteq \{0, \dots, n+k\}$ with $\{a_i, a_j\} = \{d_{U^0}(x),\, d_{U^1}(x)\}$.
%%Notice that is such $U$ exists then it is unique.
%We will now describe a condition equivalent to $(\ast)$ in terms of $\{a_i, a_j\}$ only.
%Denote
%\begin{equation*}
%\overline{a}_{i} = a_i \setminus a_j, \qquad
%\overline{a}_{j} = a_j \setminus a_i, \qquad
%\overline{a}_{ij} = \overline{a}_i \cup \overline{a}_j.
%\end{equation*}
%A necessary condition for $(\ast)$ is that $\pos_{a_{ij}} \colon \overline{a}_{ij} \to \Z$ is an isomorphism onto $U$.
%Slightly abusing notation we define the function $\ind \colon \overline{a}_{ij} \to \Ftwo$ by
%\begin{equation*}
%\ind(v) = \pos_{a_{ij}}(v) + \pos_{\overline{a}_{ij}}(v) \text{ mod }2
%\end{equation*}
%and notice that it fits in the commutative diagram
%\[
%\begin{tikzcd}[column sep=small, row sep=small]
%\overline{a}_{ij} \arrow[rr, "\pos_{a_{ij}}", "\cong"'] \arrow[dr, "\ind"', bend right] & &
%U \arrow[dl, "\ind_U", bend left] \\
%& \Ftwo &
%\end{tikzcd}
%\]
%where $\ind_U$ was introduced in \cref{d:index function}.
%Since for $\varepsilon \in \Ftwo \cong \{0,1\}$ we have $U^\varepsilon = \ind_U^{-1}(\varepsilon)$, condition $(\ast)$ is equivalent to the existence of $U$ with
%\begin{equation} \label{e:pos's equal U's}
%\big\{\pos_{a_{ij}}(\overline{a}_i),\, \pos_{a_{ij}}(\overline{a}_j)\big\} = \{U^0, U^1\}.
%\end{equation}
%Or, equivalently, that the function $\ind \colon \overline{a}_{ij} \to \Ftwo$ is constant on both $\overline{a}_i$ and $\overline{a}_j$ with different values, i.e.,
%\begin{equation*}
%\ind(\overline{a}_i) \xor \ind(\overline{a}_j) = \{0,1\},
%\end{equation*}
%where $\ind(S) = \{\ind(v) \mid v \in S\}$ for any $S \subseteq \overline{a}_{ij}$ and $S \xor S^\prime = S \cup S^\prime \setminus (S \cap S^\prime)$.
%
%\anibal{improve this last paragraph}
%There
%Therefore, for any $x \in X_{n+k}$ we have $\beta(x) = 1$ if and only if the set of pairs $\{a_i, a_j\}$ in $\pi^{-1}(x)$ with $\eval(\{a_i, a_j\}) = 1$ is odd; which is equivalent to the condition $x \in B$.
